Test-Time Adaptation via Cache Personalization for Facial Expression Recognition in Videos

Facial expression recognition (FER) in videos requires model personalization to capture considerable variation across subjects. Vision-language models (VLMs) offer strong transfer through image-text alignment, but their performance can degrade under inter-subject distribution shifts. Test-time adaptation (TTA) can mitigate this challenge, yet most state-of-the-art methods rely on unsupervised parameter optimization, introducing computational overhead that limits real-world deployment. This paper introduces TTA through Cache Personalization (TTA-CaP), a gradient-free, cache-based method for cost-effective personalization of VLMs in video FER. Unlike prior cache-based TTA methods that rely solely on dynamic memories of test samples and may drift because of noisy pseudo-labels, TTA-CaP employs three complementary caches: a personalized static cache constructed through feature-statistics matching, a positive target cache containing reliable subject-specific samples, and a negative target cache containing low-confidence cases as negative evidence. A tri-gate mechanism prevents cache corruption by controlling updates according to temporal stability, confidence, and consistency with the personalized static cache. The caches jointly provide subject-matched positive and negative evidence for robust personalization. TTA-CaP further refines predictions through embedding fusion, supporting temporally stable video-level predictions. Experiments on BioVid, StressID, and BAH show that TTA-CaP outperforms state-of-the-art TTA methods under subject-specific and environmental shifts while maintaining low computational and memory overhead. Our code is publicly available at https://github.com/MasoumehSharafi/TTA-CaP.

==> sec/2_related__work.tex <==
\section{Related  Work}
\label{sec:Related_work}



%%%%%%%%%%%
\noindent\textbf{Vision-Language Models for FER.}
VLMs trained with large-scale image--text contrastive learning, such as CLIP, enable prompt-based recognition by reframing classification as image--text matching~\cite{radford2021learning}. This is appealing for FER because expression classes are semantic; however, FER is fine-grained and entangled with identity and capture conditions, making performance sensitive to prompt design and inter-subject shifts in videos. Recent CLIP-based FER methods improve language guidance and temporal modeling. CLIPER uses multiple expression descriptors to learn more discriminative static and dynamic representations~\cite{li2024cliper}, while DFER-CLIP incorporates temporal modeling and enriched textual descriptions to better align subtle dynamics with language priors~\cite{zhao2023prompting}. In zero-shot settings, EmoCLIP uses natural-language descriptions to improve generalization~\cite{foteinopoulou2024emoclip}, and Exp-CLIP transfers task knowledge distilled from LLMs~\cite{zhao2025enhancing}. Multimodal prompt alignment and parameter-efficient adaptation further improve dynamic FER~\cite{ma2025mpafer}. However, these methods mainly focus on prompting and training-time adaptation, leaving reliable test-time adaptation for videos underexplored.


%%%%%%%%%%
\noindent\textbf{Test-Time Adaptation.}
Test-time adaptation (TTA) mitigates distribution shift by adapting a pretrained model using only unlabeled test data during inference. Early methods optimize auxiliary self-supervised or entropy-based objectives, as in test-time training, Tent, and MEMO~\cite{sun2020test,wang2020tent,zhang2022memo}. More recent approaches, including EATA, SAR, CoTTA, and RoTTA, improve stability under noisy, small-batch, or non-stationary test streams through selective updates, robust optimization, and memory mechanisms~\cite{niu2022efficient,niu2023sar,wang2022continual,yuan2023robust}. However, these methods still rely on iterative parameter updates and may suffer from confirmation bias or limited compatibility with LayerNorm-based backbones.

TTA for VLMs instead exploits CLIP's aligned image--text space and strong zero-shot priors. Methods such as TPT and PromptAlign adapt textual prompts using entropy minimization, augmented views, or feature-statistics alignment~\cite{shu2022test,abdul2023align}. Other approaches employ prompt ensembles, weight averaging, or CLIP-specific objectives to reduce pseudo-label drift and preserve image--text alignment~\cite{osowiechi2024watt,lafon2025cliptta}. Despite their effectiveness, these methods require repeated backpropagation at test time and remain sensitive to optimization choices and unreliable predictions, motivating gradient-free alternatives.

%%%%
% Cache-based approaches augment a frozen backbone with an external memory and adapt predictions via feature retrieval in embedding space~\cite{karmanov2024efficient}. In the VLM setting, CLIP-Adapter and Tip-Adapter refine CLIP predictions using lightweight adapters or non-parametric key--value caches, with Tip-Adapter-F further improving performance through fine-tuning~\cite{gao2024clip,zhang2022tip}. Training-free neighbor-based variants such as CODER also leverage neighborhood structure to improve CLIP classification~\cite{yi2024leveraging}. Recent test-time methods improve cache reliability via selective updates and calibration or prototype/statistics refinement~\cite{nguyen2025adaptivecacheenhancementtesttime,liang2025advancing,zhang2024dual,zhu2025dynamic,zhai2025mitigating,chen2025multi,chen2025paf,guanstatistics}. 
\noindent\textbf{Cache-Based TTA Methods.}
Cache-based TTA methods adapt predictions using stored target features or prototypes in the embedding space~\cite{karmanov2024efficient}. TDA~\cite{karmanov2024efficient}, DPE~\cite{zhang2024dual}, and ReTA~\cite{liang2025advancing} improve cache reliability through dynamic updates and prototype refinement, while MCP~\cite{chen2025multi} and CRG~\cite{zhai2025mitigating} exploit multiple prototypes or positive/negative evidence. In contrast, TTA-CaP is designed for subject-based video FER and combines a personalized static source cache, dynamic positive/negative target caches, temporal consistency, tri-gated updates, and embedding-level fusion. Despite these advances, existing cache-based TTA is not tailored to subject-based video FER: pseudo-label-driven target memories can degrade under frame-level noise, and most methods do not exploit subject-specific source priors to anchor class semantics, while long videos also raise memory and retrieval-cost concerns.

==> sec/6_supp_material.tex <==
\section{Table Of Contents}
\label{sec:supplementary}

\begingroup
\let\clearpage\relax
\let\newpage\relax
\let\contentsname\relax
\maketitle

\vspace{-0.5cm}

\makeatletter
\let\origcontentsline\contentsline
\def\contentsline#1#2#3#4{%
  \ifnum\pdfstrcmp{#1}{title}=0
  \else
    \ifnum\pdfstrcmp{#1}{author}=0
    \else
      \origcontentsline{#1}{#2}{#3}{#4}%
    \fi
  \fi
}
\noindent\textbf{}\par\vspace{0.3em}
\tableofcontents
\makeatother
\endgroup


% \makeatletter
% \begingroup
% \let\addcontentsline\@gobblethree
% \maketitle
% \endgroup
% \makeatother

% \vspace{+0.1cm}
% % \noindent\textbf{This supplementary material includes the following sections:}
% % \vspace{0.3cm}

% \noindent Supplementary Algorithms \dotfill 1\\
% \hspace*{1.5em} Personalized source cache construction \dotfill 2\\
% \hspace*{1.5em} Online TTA \dotfill 3\\
% Experimental Results \dotfill 1\\
% \hspace*{1.5em} TTA Baseline Methods \dotfill 1\\
% \hspace*{1.5em} Subject-Wise Results \dotfill 2\\
% \hspace*{1.5em} Ablation Studies \dotfill 3\\

% \vspace{-0.5cm}

\section{Supplementary Algorithms}
This section provides additional algorithmic details for the personalized source-prototype construction and the online test-time adaptation pipeline introduced in the main paper. In particular, we clarify how personalized source prototypes are built from the source subjects and subsequently matched to target subjects, as well as how the proposed online adaptation mechanism operates at inference time on target videos. 

Algorithm~\ref{alg:personalized_cache} describes the full procedure used to construct personalized source prototypes. Starting from source-domain embeddings, the method identifies representative subject-specific prototypes for each expression class and transfers them to a target subject through the anchor-class matching strategy described in the main paper. This procedure enables the source cache to better preserve subject-dependent structure while remaining transferable to unseen target subjects. Algorithm~\ref{alg:online_tta} summarizes the complete online test-time adaptation pipeline applied to the target video stream. It details the extraction of frame and temporal embeddings, the retrieval of evidence from the personalized source cache and target caches, the embedding-level fusion process, and the cache update mechanism based on the tri-gate rule. Together, these steps illustrate how the proposed method performs efficient and fully online personalization without updating the backbone encoders.
%%%%%%%%%%%%%%%%%%%Personalized_source_cache%%%%%%%%%%%
\begin{algorithm}[t!]
\caption{Personalized static cache}
\label{alg:personalized_cache}
\small
\KwIn{Source set $\mathcal{D}^{\mathrm{src}}$, target set $\mathcal{D}^{\mathrm{tgt}}$, frozen image encoder $E_I$, classes $\mathcal{C}$, anchor class $c_a$, top-$m$, cap $K$}
\KwOut{Personalized prototypes $\mathcal{P}^{\mathrm{pers}}_{t,c}$}

\ForEach{source subject $s$ and class $c \in \mathcal{C}$}{
    Extract normalized embeddings $\mathbf{F}_{s,c}$\;
    Select DBSCAN parameters\;
    \eIf{clustering is invalid or too few samples}{
        Set $\mathcal{M}_{s,c}$ to the sample nearest to the class mean\;
    }{
        Run DBSCAN on $\mathbf{F}_{s,c}$\;
        Set $\mathcal{M}_{s,c}$ to the medoid of each non-noise cluster\;
    }
}

\ForEach{source subject $s$}{
    Compute anchor statistics $(\mu_s^a,\tilde{\sigma}_s^{2,a})$ from $\mathcal{M}_{s,c_a}$\;
}

\ForEach{target subject $t$}{
    Compute anchor statistics $(\mu_t^a,\tilde{\sigma}_t^{2,a})$ from $\mathcal{X}_{t,c_a}$\;

    \ForEach{source subject $s$}{
        Compute anchor distance $d(s,t)$\;
    }

    Select the top-$m$ closest sources $\mathcal{S}_t$\;

    \ForEach{class $c \in \mathcal{C}$}{
        $\mathcal{P}^{\mathrm{pers}}_{t,c} \leftarrow \bigcup_{s\in\mathcal{S}_t}\mathcal{M}_{s,c}$\;
        \If{$K>0$ and $|\mathcal{P}^{\mathrm{pers}}_{t,c}|>K$}{
            Keep the $K$ most relevant prototypes\;
        }
    }
}

\Return{$\{\mathcal{P}^{\mathrm{pers}}_{t,c}\}_{t,c}$}\;
\end{algorithm}

%%%%%%%%%%%%%%%online TTA%%%%%%%%%%%%%%%
\begin{algorithm}[t!]
\caption{\ours: online TTA}
\label{alg:online_tta}
\small
\DontPrintSemicolon
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}

\Input{Target video $\mathcal{V}^{\mathrm{tgt}}_t=\{x^{\mathrm{tgt}}_t\}_{t=1}^{T}$; frozen image encoder $E_I$; frozen temporal encoder $E_t$; frozen text encoder $E_T$; class prompts $\{\tau_c\}_{c\in\mathcal C}$; personalized source cache $\mathcal P^{\mathrm{src,tgt}}$; target caches $C^{\mathrm{tgt}+}, C^{\mathrm{tgt}-}$.}
\Output{Video prediction $\hat y$; updated target caches $C^{\mathrm{tgt}+}, C^{\mathrm{tgt}-}$.}

\ForEach{$c\in\mathcal C$}{
    Compute normalized text embedding $e_c \leftarrow E_T(\tau_c)$\;
}

\For{$t=1$ \KwTo $T$}{
    Extract frame embedding $h_t \leftarrow E_I(x_t)$\;
    Compute temporal target embedding
    $z_t^{\mathrm{tgt}} \leftarrow \textsc{Pool}(E_t(h_{t-W+1:t}))$\;
    Normalize $z_t^{\mathrm{tgt}}$\;

    \ForEach{$c\in\mathcal C$}{
        $\ell_t^{\mathrm{base}}(c) \leftarrow \eta \cdot \cos(z_t^{\mathrm{tgt}}, e_c)$\;
    }
    $\tilde y_t \leftarrow \arg\max_{c\in\mathcal C}\ell_t^{\mathrm{base}}(c)$\;
    Compute current-frame entropy $h^\text{tgt}_k$\;

    $(C^{\mathrm{tgt}+}, C^{\mathrm{tgt}-}) \leftarrow
    \textsc{TriGateUpdate}(z_k^{\mathrm{tgt}}, \tilde{y}^\text{tgt}_k, h^\text{tgt}_k, \mathcal P^{\mathrm{src,tgt}}, C^{\mathrm{tgt}+}, C^{\mathrm{tgt}-})$\;

    Retrieve source and target cache evidence:
    $z_t^{\mathrm{src,tgt}} \leftarrow \textsc{RetrieveSrc}(\mathcal P^{\mathrm{src,tgt}}, z_t^{\mathrm{tgt}})$,
    $z_t^{\mathrm{tgt}+} \leftarrow \textsc{RetrievePos}(C^{\mathrm{tgt}+}, z_t^{\mathrm{tgt}})$,
    $z_t^{\mathrm{tgt}-} \leftarrow \textsc{RetrieveNeg}(C^{\mathrm{tgt}-}, z_t^{\mathrm{tgt}})$\;

    $z_t^{\mathrm{fuse}} \leftarrow z_t^{\mathrm{tgt}} + z_t^{\mathrm{src,tgt}} + z_t^{\mathrm{tgt}+} - z_t^{\mathrm{tgt}-}$\;
    Normalize $z_t^{\mathrm{fuse}}$\;

    \ForEach{$c\in\mathcal C$}{
        $\ell_t(c) \leftarrow \eta \cdot \cos(z_t^{\mathrm{fuse}}, e_c)$\;
    }
}

$\hat y \leftarrow \arg\max_{c\in\mathcal C}\frac{1}{T}\sum_{t=1}^{T}\ell_t(c)$\;

\Return{$\hat y, C^{\mathrm{tgt}+}, C^{\mathrm{tgt}-}$}\;
\end{algorithm}

\section{Experimental Results}

\subsection{TTA Baseline Methods}
We compare against several CLIP-based test-time adaptation baselines. \emph{TPT}~\cite{shu2022test} updates only the textual prompt tokens during inference by minimizing prediction entropy over strongly augmented views, while keeping both the image and text encoders frozen. \emph{TDA}~\cite{karmanov2024efficient} is a training-free dynamic adapter that builds a feature--label cache online, progressively refines pseudo-labels, including negative pseudo-labels, and combines cache-based predictions with CLIP zero-shot logits. \emph{DPE}~\cite{zhang2024dual} updates visual and textual class prototypes jointly at test time, introduces lightweight sample-specific residuals, and encourages cross-modal consistency between the two prototype spaces under distribution shift. \emph{PromptAlign}~\cite{abdul2023align} adapts prompts by aligning test-time feature statistics with source-domain statistics, thereby reducing distribution mismatch beyond standard entropy-minimization objectives. \emph{ReTA}~\cite{liang2025advancing} emphasizes reliable cache-based VLM adaptation through CER (consistency-aware entropy reweighting) for selective cache updates and DDC (diversity-driven distribution calibration), which models each class as a Gaussian family over evolving text embeddings to improve calibration. Finally, \emph{T3AL}~\cite{liberatori2024test}, originally proposed for zero-shot temporal action localization, is adapted here for classification by using video-level pseudo-labels from aggregated frame features, self-supervised refinement of frame-level predictions, and text-guided suppression of irrelevant regions, while keeping the encoders frozen and resetting updates for each sample.

\subsection{Subject-Wise Results}

Tabs.~\ref{tab:biovid_subject_war}, \ref{tab:stressid_subject_war}, and \ref{tab:bah_subject_war} report the subject-wise performance across the ten target subjects for each dataset. Each experiment was repeated three times to assess reliability, and the tables report the mean performance with standard deviation over these three trials. These results provide a detailed view of the robustness of each method under subject-level distribution shifts.

On \biovid, most baseline methods show strong performance on certain subjects but suffer noticeable degradation on others, reflecting the difficulty of adapting to individual expression patterns. In contrast, \ours consistently improves performance for most subjects and achieves the highest overall average score. The gains are particularly visible for subjects where baseline methods exhibit larger performance gaps. A similar trend is observed on \stressid, where subject-specific variability is more pronounced. While baseline methods often fluctuate substantially across subjects, \ours maintains more stable performance and obtains the best average \war and \uar scores. For \bah, the improvements are more moderate due to the dataset's higher difficulty and the limited discriminative signal reflected in the \uar scores. Nevertheless, \ours still achieves the best average \war among all methods while maintaining competitive \uar results. Overall, these subject-wise analyses highlight the benefits of the proposed personalized cache construction and tri-gate update strategy, which enables \ours to better adapt to subject-specific characteristics at test time.

\subsection{Ablation Studies}

\noindent\textbf{Embedding vs.\ logit fusion.}
Fig.~\ref{fig:reliability_diag} reports video-level calibration using reliability diagrams for logit-space and embedding-space fusion. Both curves deviate from the diagonal reference, indicating residual miscalibration, while the curve closer to the diagonal corresponds to better alignment between confidence and empirical accuracy, i.e., lower expected calibration error (ECE)~\cite{guo2017calibration}. This comparison highlights how the choice of fusion space affects not only recognition performance but also the reliability of confidence estimates used for downstream decision-making.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%biovid%%%%%%%%%%%%%%%%%%

\begin{table*}[t!]
\centering
\scriptsize

% \footnotesize
% \setlength{\tabcolsep}{3pt}
\resizebox{0.9\linewidth}{!}{%
\begin{tabular}{l|cccccccccc|c}
\toprule
\textbf{Method} & Sub-1 & Sub-2 & Sub-3 & Sub-4 & Sub-5 & Sub-6 & Sub-7 & Sub-8 & Sub-9 & Sub-10 & Avg. \\
\midrule
TPT          & 91.9\std{0.12} & 53.0\std{0.31} & 50.0\std{0.00} & 61.5\std{0.36} & 79.0\std{0.19} & 88.9\std{0.14} & 76.0\std{0.12} & 50.0\std{0.00} & 98.9\std{0.05} & 62.0\std{0.28} & 71.1 \\
TDA          & 93.0\std{0.10} & 52.6\std{0.29} & 50.0\std{0.00} & 63.9\std{0.32} & 79.5\std{0.17} & 87.5\std{0.16} & 76.3\std{0.18} & 50.0\std{0.00} & 100.0\std{0.00} & 61.6\std{0.26} & 71.4 \\
DPE          & 91.7\std{0.13} & 55.0\std{0.27} & 50.0\std{0.00} & 85.0\std{0.18} & 73.0\std{0.24} & 84.7\std{0.20} & 80.0\std{0.16} & 50.0\std{0.00} & 100.0\std{0.00} & 61.8\std{0.20} & 73.1 \\
PromptAlign  & 93.8\std{0.09} & 65.2\std{0.21} & 50.0\std{0.00} & 70.0\std{0.24} & 85.0\std{0.14} & 92.0\std{0.10} & 80.0\std{0.15} & 50.0\std{0.00} & 100.0\std{0.00} & 67.6\std{0.20} & 75.3 \\
ReTA         & 93.8\std{0.08} & 65.2\std{0.19} & 50.0\std{0.00} & 69.5\std{0.22} & 85.0\std{0.13} & 90.2\std{0.12} & 80.0\std{0.14} & 50.0\std{0.00} & 100.0\std{0.00} & 67.6\std{0.18} & 75.1 \\
T3AL         & 94.0\std{0.07} & 66.5\std{0.18} & 50.0\std{0.00} & 70.0\std{0.21} & 85.2\std{0.12} & 94.2\std{0.08} & 83.9\std{0.13} & 50.0\std{0.00} & 100.0\std{0.00} & 67.6\std{0.17} & 76.1 \\
\rowcolor{pinkTTA}
\textbf{\ours} & 95.0\std{0.09} & 75.0\std{0.16} & 50.0\std{0.00} & 100.0\std{0.00} & 92.5\std{0.10} & 97.5\std{0.06} & 92.5\std{0.09} & 50.0\std{0.00} & 100.0\std{0.00} & 62.5\std{0.19} & \textbf{81.5} \\

\bottomrule
\end{tabular}%
 }

\caption{Subject-wise \war score on the \biovid dataset for \ours and competing TTA methods. Best results are shown in \textbf{bold}.}
\label{tab:biovid_subject_war}
% \vspace{0.3em}
\end{table*}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%stressid%%%%%%%%%%%%%%%%%%%
\begin{table*}[t!]
\centering
\scriptsize

% \footnotesize
% \setlength{\tabcolsep}{3pt}
\resizebox{0.9\linewidth}{!}{%
\begin{tabular}{l|cccccccccc|c}
\toprule
\textbf{Method} & Sub-1 & Sub-2 & Sub-3 & Sub-4 & Sub-5 & Sub-6 & Sub-7 & Sub-8 & Sub-9 & Sub-10 & Avg. \\
\midrule
TPT         & 74.7\std{0.18} & 51.6\std{0.21} & 90.0\std{0.09} & 88.0\std{0.12} & 52.2\std{0.24} & 77.5\std{0.11} & 66.6\std{0.22} & 63.4\std{0.19} & 54.0\std{0.23} & 91.9\std{0.08} & 70.9 \\
TDA         & 66.9\std{0.22} & 45.2\std{0.28} & 75.6\std{0.17} & 90.1\std{0.10} & 49.6\std{0.24} & 80.0\std{0.05} & 41.2\std{0.31} & 75.3\std{0.18} & 81.8\std{0.02} & 91.9\std{0.07} & 69.7 \\
DPE         & 64.0\std{0.23} & 55.0\std{0.20} & 73.9\std{0.18} & 90.0\std{0.09} & 52.6\std{0.22} & 80.0\std{0.05} & 50.9\std{0.27} & 73.0\std{0.19} & 81.8\std{0.07} & 92.0\std{0.07} & 71.3 \\
PromptAlign & 69.9\std{0.20} & 61.6\std{0.17} & 78.6\std{0.14} & 90.9\std{0.08} & 51.2\std{0.21} & 80.0\std{0.15} & 60.4\std{0.19} & 81.3\std{0.13} & 81.8\std{0.06} & 90.9\std{0.09} & 74.6 \\
ReTA        & 64.5\std{0.21} & 50.5\std{0.23} & 82.0\std{0.12} & 90.0\std{0.09} & 46.8\std{0.25} & 80.0\std{0.12} & 49.3\std{0.29} & 80.0\std{0.04} & 81.8\std{0.10} & 93.7\std{0.06} & 71.8 \\
T3AL        & 71.3\std{0.18} & 62.7\std{0.16} & 80.3\std{0.13} & 90.2\std{0.08} & 54.0\std{0.20} & 80.0\std{0.07} & 68.0\std{0.17} & 77.0\std{0.14} & 82.0\std{0.05} & 93.9\std{0.06} & 75.9 \\
\rowcolor{pinkTTA}
\textbf{\ours} & 83.3\std{0.14} & 66.6\std{0.15} & 90.0\std{0.08} & 88.8\std{0.10} & 75.0\std{0.16} & 82.2\std{0.09} & 69.9\std{0.18} & 82.0\std{0.07} & 83.4\std{0.06} & 94.0\std{0.05} & \textbf{81.5} \\


\bottomrule
\end{tabular}%
 }

\caption{Subject-wise \war score on the \stressid dataset for \ours and competing TTA methods.}
\label{tab:stressid_subject_war}
% \vspace{0.3em}
\end{table*}

\begin{table*}[t!]
\centering
\scriptsize

% \footnotesize
% \setlength{\tabcolsep}{3pt}
\resizebox{0.9\linewidth}{!}{%
\begin{tabular}{l|cccccccccc|c}
\toprule
\textbf{Method} & Sub-1 & Sub-2 & Sub-3 & Sub-4 & Sub-5 & Sub-6 & Sub-7 & Sub-8 & Sub-9 & Sub-10 & Avg. \\
\midrule
TPT         & 62.0\std{0.18} & 53.7\std{0.19} & 73.9\std{0.14} & 80.0\std{0.11} & 81.2\std{0.10} & 71.0\std{0.16} & 58.0\std{0.17} & 55.0\std{0.18} & 69.0\std{0.15} & 53.0\std{0.20} & 65.6 \\
TDA         & 58.0\std{0.20} & 53.7\std{0.18} & 75.0\std{0.13} & 80.3\std{0.10} & 79.0\std{0.12} & 71.6\std{0.15} & 58.0\std{0.16} & 55.9\std{0.17} & 69.0\std{0.14} & 51.7\std{0.22} & 65.2 \\
DPE         & 58.6\std{0.19} & 59.6\std{0.16} & 79.6\std{0.10} & 80.5\std{0.10} & 83.4\std{0.09} & 67.0\std{0.18} & 59.0\std{0.15} & 54.0\std{0.19} & 71.9\std{0.12} & 54.0\std{0.18} & 66.7 \\
PromptAlign & 59.1\std{0.18} & 59.1\std{0.16} & 72.0\std{0.15} & 84.5\std{0.09} & 84.1\std{0.08} & 72.4\std{0.14} & 58.5\std{0.16} & 55.9\std{0.17} & 71.5\std{0.12} & 54.9\std{0.17} & 67.1 \\
ReTA        & 61.4\std{0.17} & 60.0\std{0.15} & 72.0\std{0.14} & 84.0\std{0.09} & 84.1\std{0.08} & 72.4\std{0.13} & 58.5\std{0.15} & 55.9\std{0.16} & 72.0\std{0.11} & 56.0\std{0.16} & 67.6 \\
T3AL        & 61.0\std{0.17} & 58.9\std{0.16} & 75.0\std{0.13} & 85.6\std{0.08} & 83.6\std{0.09} & 74.7\std{0.12} & 60.0\std{0.14} & 56.0\std{0.15} & 71.0\std{0.12} & 53.6\std{0.18} & 67.9 \\
\rowcolor{pinkTTA}
\textbf{\ours} & 62.5\std{0.16} & 62.1\std{0.14} & 79.6\std{0.09} & 85.8\std{0.07} & 84.4\std{0.08} & 75.2\std{0.11} & 60.1\std{0.13} & 56.6\std{0.14} & 70.0\std{0.13} & 56.6\std{0.15} & \textbf{69.2} \\

\bottomrule
\end{tabular}%
 }

\caption{Subject-wise \war score on the \bah dataset for \ours and competing TTA methods.}
\label{tab:bah_subject_war}
% \vspace{0.3em}
\end{table*}

\noindent\textbf{Class prompt selection.}
An ablation study was conducted on a diverse set of class-prompt templates commonly used in CLIP-based FER and prompt-based recognition settings~\cite{foteinopoulou2024emoclip, ni2022expanding, zhao2025enhancing}. The goal is to assess how the wording of emotion-class prompts affects the quality of text representations and, in turn, downstream recognition performance. These results are obtained using CLIP ViT-B/32, trained on the \biovid source subjects and evaluated on the target subjects. As shown in Tab.~\ref{tab:class_prompt_ablation_full}, prompt design has a noticeable impact on both \war and \fonescore score. Among the evaluated templates, \emph{``a person with an expression of [CLS]''} yields the best overall performance and is therefore adopted in all methods that rely on class prompts.

%%%%%%%%%%%%%%%%%%%%%Class-prompts%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.1}
\caption{Ablation of class-prompt templates for the CLIP text encoder on \biovid using CLIP ViT-B/32. Performance varies noticeably across prompt formulations, and the template \emph{“a person with an expression of [CLS]”} achieves the best \war and \fonescore score.}
\begin{tabular}{lcc}
\toprule
\textbf{Prompt Template} & \textbf{\war} & \textbf{\fonescore score} \\
\midrule
a photo of a [CLS]                                      & 68.7 & 63.3 \\
a\_photo\_of\_the\_[CLS]\_face                          & 66.5 & 59.3 \\
a\_photo\_of\_one\_[CLS]\_face                          & 64.2 & 55.8 \\
a\_close-up\_photo\_of\_the\_[CLS]\_face                & 68.2 & 62.6 \\
a\_low\_resolution\_photo\_of\_a\_[CLS]\_face           & 68.7 & 64.2 \\
a\_good\_photo\_of\_a\_[CLS]\_face                      & 69.2 & 65.4 \\
a\_photo\_of\_my\_[CLS]\_face                           & 66.2 & 60.3 \\
a\_cropped\_photo\_of\_the\_[CLS]\_face                 & 64.5 & 57.5 \\
a\_photo\_of\_a\_person\_with\_[CLS]\_face              & 67.2 & 61.4 \\
\rowcolor{pinkTTA}
\textbf{a person with an expression of [CLS]}           & \textbf{69.7} & \textbf{66.6} \\
a\_portrait\_of\_a\_person\_in\_[CLS]                   & 58.2 & 46.7 \\
a\_face\_showing\_signs\_of\_[CLS]                      & 68.7 & 64.1 \\
a close up portrait of a [CLS] expression               & 69.2 & 63.0 \\
a realistic photo of a person experiencing [CLS]        & 53.5 & 40.0 \\
a cropped image of a person in [CLS]                    & 69.0 & 64.5 \\
a photo of a [CLS] person                               & 69.5 & 64.3 \\
a person with a facial expression of [CLS]              & 69.5 & 64.2 \\
a high quality photo of a [CLS] expression              & 69.5 & 64.3 \\
a photo of a face showing [CLS]                         & 69.5 & 64.3 \\
a photo of a face in [CLS]                              & 69.0 & 61.8 \\
\bottomrule
\end{tabular}
\label{tab:class_prompt_ablation_full}
\end{table}


\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\caption{Calibration and performance comparison on \biovid.}
\label{tab:ece_calibration}
\begin{tabular}{lcc}
\toprule
\textbf{Method} & \textbf{Logit ECE} $\downarrow$ & \textbf{Embed ECE} $\downarrow$ \\
\midrule
TDA  & 20.7 & 15.2 \\
ReTA & 19.2 & 14.0 \\
\ours  & \textbf{17.8} & \textbf{12.3} \\
\bottomrule
\end{tabular}
\end{table}

%%%%%%%%%RIGHT TABLE MOVED HERE%%%%%%%%%%%%%%%
\begin{table}[t!]
\centering
\small
\setlength{\tabcolsep}{6pt}
\caption{Effect of different static source-cache construction strategies. Average \war{} (\%) over target subjects in \biovid using \ours{}.}
\label{tab:src_cache_build}
\begin{tabular}{lc}
\toprule
\textbf{Cache construction} & \textbf{\war(\%)} $\uparrow$ \\
\midrule
Baseline (k-means, $k{=}1$) & 78.8 \\
Two-stage (k-means) & 79.3 \\
Two-stage (DBSCAN) & 79.5 \\
Personalized (k-means) & 79.6 \\
Personalized (DBSCAN) & \textbf{81.0} \\
\bottomrule
\end{tabular}
\end{table}

\noindent\textbf{Ablation on personalized static cache construction}
Alternative strategies for constructing the static personalized source cache are compared while keeping the online TTA pipeline and cache budget fixed. As a simple baseline, a single prototype is selected per (subject, class) by applying k-means clustering~\cite{lloyd1982least, mcqueen1967some} with $k{=}1$ (i.e., the closest sample to the class centroid). Next, a two-stage clustering strategy is evaluated, where prototypes are first selected per (subject, class) and then re-clustered after pooling across subjects to produce a compact class-level cache; both k-means and DBSCAN~\cite{ester1996density} are considered in this second clustering step. Finally, fully personalized prototype selection is considered by retaining subject-specific clusters (k-means/DBSCAN) instead of pooling across subjects. 
Tab.~\ref{tab:src_cache_build} shows that increasing prototype diversity and personalization consistently improves \war: the $k{=}1$ baseline achieves 78.8 \war, two-stage clustering provides modest gains (79.3--79.5), and personalized clustering yields further improvements, with personalized DBSCAN achieving the best result of 81.7 \war. Overall, the results indicate that preserving subject-specific structure in the source cache is beneficial under domain shift.

\noindent\textbf{Ablation on Cache Weighting.} Tab.~\ref{tab:fusion_ablation} compares three strategies for combining the predictions of the personalized source, positive target, and negative target caches. Equal-weight fusion assigns the same contribution to each cache, confidence-weighted fusion scales each cache according to its prediction confidence, and attention-based fusion estimates sample-dependent cache weights using a learned attention module. Equal-weight fusion achieves the best performance of 81.0\% \war, outperforming confidence-weighted and attention-based fusion by 2.1 and 3.6 percentage points, respectively. This result suggests that uniform aggregation provides a more stable balance among the complementary cache signals, whereas adaptive weighting may overemphasize noisy or overconfident predictions.

\begin{table}[t!]
\centering
\setlength{\tabcolsep}{8pt}
\scriptsize
\renewcommand{\arraystretch}{1.15}
\setlength{\tabcolsep}{7pt}
\begin{tabular}{lr}
\toprule
\textbf{Weighting Strategy} & \textbf{\war\ (\%)} $\uparrow$ \\
\midrule
Conf.-weighted  & 78.9 \\
Attention-based & 77.4 \\
Equal-weight    & \textbf{81.0} \\
\bottomrule
\end{tabular}
\caption{Ablation of cache-weighting strategies on \biovid.
Results report the average \war over target subjects.}
\label{tab:fusion_ablation}
\end{table}

\noindent\textbf{Static Cache Generation Strategy.}
The effect of source cache without using source data construction is analyzed under the same online TTA pipeline and cache budget. We studied four different methods to build the static cache prototypes: (i) GMM virtual prototypes sampled around class centers (classifier-weight anchors), (ii) random sampling in the embedding space with pseudo-labeling by the frozen classifier, (iii) classifier prototypes using the classifier weights directly as class anchors, and (iv) a generator-based feature-space model that produces class-conditional avatar prototypes. Fig.~\ref{fig:src_cache_gen_war} shows that more class-consistent source prototypes yield stronger downstream adaptation: the generator-based source cache performs best among data-free strategies (\war= 79.1), while GMM perturbations around class centers are less effective (\war = 74.0). For comparison, the full \ours configuration with personalized source-subject prototypes (“Prototypes” in the figure) achieves \war=81.0, indicating that higher-quality source prototypes provide a strong foundation and are further strengthened when combined with the complete cache design.

%%%%%%%%%%%%%%%%%%%%%%ablation_each_cache_and_generated%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t!]
  \centering
  \begin{subfigure}{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{cache_ablation_bar.png}
    \caption{}
    \label{fig:cache_ablation_bar}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{src_cache_gen_war.png}
    \caption{}
    \label{fig:src_cache_gen_war}
  \end{subfigure}
  \caption{\textbf{(a)} Average \war for target subjects in \biovid for zero-shot CLIP, static personalized source cache only, dynamic target cache only, and \ours (static + dynamic). \textbf{(b)} Ablation of source-cache construction in \biovid. Average \war across target subjects. Prototypes: the personalized source cache built from source-subject prototypes.}
  \label{fig:ablation_biovid_bars}
\end{figure}
